SZZ in the time of Pull Requests

In the multi-commit development model, programmers complete tasks (e.g., implementing a feature) by organizing their work in several commits and packaging them into a commit-set. Analyzing data from developers using this model can be useful to tackle challenging developers' needs, such as knowing which features introduce a bug as well as assessing the risk of integrating certain features in a release. However, to do so one first needs to identify fix-inducing commit-sets. For such an identification, the SZZ algorithm is the most natural candidate, but its performance has not been evaluated in the multi-commit context yet. In this study, we conduct an in-depth investigation on the reliability and performance of SZZ in the multi-commit model. To obtain a reliable ground truth, we consider an already existing SZZ dataset and adapt it to the multi-commit context. Moreover, we devise a second dataset that is more extensive and directly created by developers as well as Quality Assurance (QA) engineers of Mozilla. Based on these datasets, we (1) test the performance of B-SZZ and its non-language-specific SZZ variations in the context of the multi-commit model, (2) investigate the reasons behind their specific behavior, and (3) analyze the impact of non-relevant commits in a commit-set and automatically detect them before using SZZ.

==> img/feature_corr.tex <==
\begin{figure}[h]
	\centering
	\includegraphics[width=8cm]{img/feature_correlation.pdf}
	\caption{Correlation among the considered features in the \mozillab}
	\label{fig:feature_corr}
\end{figure}





==> img/gt_workflow.tex <==
 \begin{figure*}[ht]
 	\includegraphics[width=\linewidth]{img/gt_workflow2.pdf}
 	\caption{Workflow of Ground Truth building. In the example, a deployed feature (on the left) [\textit{\protect\url{https://bugzilla.mozilla.org/show_bug.cgi?id=1618202}}] introduced a bug. Once discovered, the reviewer opened an issue (on the right) [\textit{\protect\url{https://bugzilla.mozilla.org/show_bug.cgi?id=1622113}}] identifying where the bug has been introduced. So, it updates the references applying the flags \textit{Regressions} to the issue associated to the bug-introducing pull request and \textit{Regressed by} to the new issue aimed to solve that bug. In this way, once the fix is published, we are able to recover the bug-introducing (in red) and fix-introducing (in green) pull requests.}
 	\label{fig:gt_workflow}
 	
\end{figure*}


==> img/i_o_algorothm.tex <==

\begin{algorithm}
	\caption{Evaluating SZZ at PR-Level with I/O Strategies}
	\label{prszz_algo:i_o_strategies}
	\begin{algorithmic} 
		\STATE $PR_{fix} \leftarrow \{c_x, c_{x+1}, ..., c_{x+n}\}$
		\STATE $PR_{bug} \leftarrow \{c_y, c_{y+1}, ..., c_{y+m}\}$
		\STATE $RES_{PR_{fix}} \leftarrow \emptyset$
		\STATE $T_{input}(PR_{fix}) = C_{fix} \leftarrow filter(PR_{fix},\space input\_strategy)$
		\FOR{\textbf{all} $c \in C_{fix}$}
		\STATE \textbf{run} $SZZ(c)$
		\STATE \textbf{add} SZZ output to $RES_{PR_{fix}}$
		\ENDFOR
		\STATE $flag(PR_i) \leftarrow match(RES_{PR_i}, \space PR_{bug},\space output\_strategy)$
		\IF{$flag = true$}
		\STATE \textbf{accept} $RES_{PR_{fix}}$
		\ELSE
		\STATE \textbf{reject} $RES_{PR_{fix}}$
		\ENDIF
	\end{algorithmic}
\end{algorithm}

==> img/i_o_strategies.tex <==
\begin{figure}[ht]
	\includegraphics[width=0.9\linewidth]{img/o_strategies.pdf}
	\caption{Output Strategies}
	\label{fig:szz_o_strategies}
	
\end{figure}

==> img/input_strategies.tex <==
\begin{figure}[ht]
	\includegraphics[width=\linewidth]{img/i_strategies.pdf}
	\caption{Input Strategies}
	\label{fig:szz_i_strategies}	
\end{figure}

==> img/output_strategies.tex <==
\begin{figure}[ht]
	\includegraphics[width=0.9\linewidth]{img/o_strategies.pdf}
	\caption{Output Strategies}
	\label{fig:szz_o_strategies}
	
\end{figure}

==> img/pca.tex <==
\begin{figure*}[h]
	\centering
	\includegraphics[width=8cm]{img/pca.png}
	\caption{Principal Component Analysis \mozilla dataset}
	\label{fig:pca}
\end{figure*}





==> img/pr_del_box.tex <==
\begin{figure}[h]
	\centering
	\includegraphics[width=8cm]{img/deletion.pdf}
	\caption{Feature Correlation in \mozilla dataset}
	\label{fig:pr_del_box}
\end{figure}





==> tables/existing_datasets.tex <==
\begin{table}[ht]	
	\begin{center}
		\caption{Existing Datasets built with SZZ}
		\label{tab:existing_dataset}

		\begin{tabular}{|l c c r|}
			\hline	
			\textbf{Dataset} & \textbf{Type} & \textbf{Languages} & \textbf{Year} \\
			ECLIPSE \cite{zimmermann2007predicting} & Open Source & Java & 2007 \\
			AEEEM \cite{d2012evaluating}& Open Source & Java & 2012 \\
			NETGENE \cite{herzig2013predicting} & Open Source & Java & 2013 \\
			JIT \cite{kamei2012large} & Open Source & Java, Perl, C++, Ruby & 2013 \\
			AUDI \cite{altinger2015novel} & Proprietary & C & 2015 \\
			SHIPPEY \cite{shippey2016so} & Open Source & Java & 2016 \\ 
			GITHUB \cite{toth2016public} & Open Source & Java & 2016 \\ 
			FJIT \cite{pascarella2019} & Open Source & Java, JavaScript, Perl, C & 2019 \\
			\hline
		\end{tabular}
	\end{center}

\end{table}

==> tables/io_strategies.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[ht]
	\centering
	\caption{SZZ Performances on Pull Request level with different I/O Strategies}
	\label{tab:szz_io}
	\begin{tabular}{|c|l|rrr|rrr|rrr|rrr|}
		\hline
		 
		 &
		\multicolumn{1}{c|}{} &
		\multicolumn{12}{c|}{Output Strategy} \\ \cline{3-14} 
		 
		 &
		\multicolumn{1}{c|}{} &
		\multicolumn{3}{c|}{All Correct} &
		\multicolumn{3}{c|}{At Least One Correct} &
		\multicolumn{3}{c|}{Positive Subset} &
		\multicolumn{3}{c|}{Majority Vote} \\ \cline{3-14} 
		 
		\multirow{-3}{*}{Variation} &
		\multicolumn{1}{c|}{\multirow{-3}{*}{Input Strategy}} &
		\multicolumn{1}{c|}{Prec.} &
		\multicolumn{1}{c|}{Recall} &
		\multicolumn{1}{c|}{F1} &
		\multicolumn{1}{c|}{Prec.} &
		\multicolumn{1}{c|}{Recall} &
		\multicolumn{1}{c|}{F1} &
		\multicolumn{1}{c|}{Prec.} &
		\multicolumn{1}{c|}{Recall} &
		\multicolumn{1}{c|}{F1} &
		\multicolumn{1}{c|}{Prec.} &
		\multicolumn{1}{c|}{Recall} &
		\multicolumn{1}{c|}{F1} \\ \hline
		 &
		One by One &
		0.118 &
		0.094 &
		0.104 &
		0.468 &
		0.373 &
		0.415 &
		0.286 &
		0.228 &
		0.254 &
		0.420 &
		0.320 &
		0.363 \\
		 
		 &
		Oldest Commit&
		0.136 &
		0.103 &
		0.117 &
		0.458 &
		0.347 &
		0.395 &
		0.278 &
		0.211 &
		0.240 &
		0.453 &
		0.349 &
		0.394 \\
		 &
		Largest Commit&
		0.131 &
		0.101 &
		0.114 &
		0.453 &
		0.349 &
		0.394 &
		0.276 &
		0.212 &
		0.240 &
		0.453 &
		0.349 &
		0.394 \\
		 
		\multirow{-4}{*}{AG} &
		Majority Files &
		0.118 &
		0.094 &
		0.105 &
		0.465 &
		0.371 &
		0.413 &
		0.285 &
		0.227 &
		0.253 &
		0.419 &
		0.320 &
		0.363 \\ \hline
		 &
		One by One &
		0.107 &
		0.090 &
		0.098 &
		0.573 &
		0.483 &
		0.524 &
		0.359 &
		0.302 &
		0.328 &
		0.509 &
		0.413 &
		0.456 \\
		 
		 &
		Oldest Commit &
		0.121 &
		0.098 &
		0.108 &
		0.554 &
		0.450 &
		0.496 &
		0.344 &
		0.279 &
		0.308 &
		0.554 &
		0.450 &
		0.496 \\
		 &
		Largest Commit &
		0.116 &
		0.095 &
		0.105 &
		0.550 &
		0.452 &
		0.496 &
		0.343 &
		0.282 &
		0.309 &
		0.550 &
		0.452 &
		0.496 \\
		 
		\multirow{-4}{*}{B} &
		Majority Files &
		0.107 &
		0.090 &
		0.098 &
		0.569 &
		0.479 &
		0.520 &
		0.356 &
		0.300 &
		0.326 &
		0.509 &
		0.414 &
		0.457 \\ \hline
		 &
		One by One &
		0.131 &
		0.100 &
		0.113 &
		0.343 &
		0.263 &
		0.298 &
		0.213 &
		0.163 &
		0.184 &
		0.357 &
		0.284 &
		0.316 \\
		 
		 &
		Oldest Commit&
		0.133 &
		0.101 &
		0.115 &
		0.347 &
		0.266 &
		0.301 &
		0.215 &
		0.164 &
		0.186 &
		0.347 &
		0.266 &
		0.301 \\
		 &
		Largest Commit&
		0.131 &
		0.100 &
		0.113 &
		0.343 &
		0.263 &
		0.298 &
		0.213 &
		0.163 &
		0.184 &
		0.343 &
		0.263 &
		0.298 \\
		 
		\multirow{-4}{*}{L} &
		Majority Files &
		0.131 &
		0.096 &
		0.111 &
		0.342 &
		0.249 &
		0.288 &
		0.211 &
		0.153 &
		0.178 &
		0.342 &
		0.249 &
		0.288 \\ \hline
		 &
		One by One &
		0.168 &
		0.133 &
		0.148 &
		0.467 &
		0.370 &
		0.413 &
		0.285 &
		0.226 &
		0.252 &
		0.447 &
		0.323 &
		0.375 \\
		 
		 &
		Oldest Commit&
		0.179 &
		0.136 &
		0.155 &
		0.449 &
		0.341 &
		0.388 &
		0.270 &
		0.205 &
		0.233 &
		0.449 &
		0.341 &
		0.388 \\
		 &
		Largest Commit&
		0.179 &
		0.136 &
		0.155 &
		0.452 &
		0.344 &
		0.390 &
		0.273 &
		0.208 &
		0.236 &
		0.452 &
		0.344 &
		0.390 \\
		 
		\multirow{-4}{*}{R} &
		Majority Files &
		0.169 &
		0.134 &
		0.149 &
		0.466 &
		0.368 &
		0.411 &
		0.284 &
		0.224 &
		0.251 &
		0.447 &
		0.324 &
		0.376 \\ \hline
		 &
		One by One &
		0.107 &
		0.089 &
		0.097 &
		0.574 &
		0.480 &
		0.523 &
		0.360 &
		0.301 &
		0.328 &
		0.515 &
		0.414 &
		0.459 \\
		 
		 &
		Oldest Commit&
		0.121 &
		0.097 &
		0.108 &
		0.556 &
		0.445 &
		0.494 &
		0.277 &
		0.345 &
		0.307 &
		0.556 &
		0.445 &
		0.494 \\
		 &
		Largest Commit&
		0.116 &
		0.094 &
		0.104 &
		0.551 &
		0.448 &
		0.494 &
		0.344 &
		0.280 &
		0.308 &
		0.551 &
		0.448 &
		0.494 \\
		 
		\multirow{-4}{*}{PD} &
		Majority Files&
		0.107 &
		0.089 &
		0.097 &
		0.570 &
		0.476 &
		0.519 &
		0.357 &
		0.298 &
		0.325 &
		0.516 &
		0.415 &
		0.460 \\ \hline
	\end{tabular}
\end{table*}

==> tables/jaccard_distance.tex <==
\begin{table}[t]
	\begin{center}
		
		\caption{SZZ Average Jaccard Distances}
		\label{tab:szz_jaccard_distance}
		{\rowcolors{2}{LightCyan}{white}
		\begin{tabular}{|l|c|c|}
			\hline
			\textbf{Algorithm} & \textbf{Commit-Set Level} & \textbf{Commit Level}\\
			\hline\hline
			\textbf{B-SZZ} & 0.81 & 0.65 \\
			\textbf{AG-SZZ} & 0.82 & 0.66 \\ 
			\textbf{L-SZZ} & 0.84 & 0.70 \\ 
			\textbf{R-SZZ} & 0.80 & 0.61 \\ 
			\textbf{Pydriller} & 0.81 & 0.65 \\ 
			\hline
		\end{tabular}
		}
	\end{center}		
\end{table}

==> tables/pca_results.tex <==
\begin{table}[t]
	\begin{center}
		
		\caption{Principal Component Analysis}
		\label{tab:szz_ml_performances}
		\begin{tabular}{|l|r|}
			\hline
			\textbf{Feature} & \textbf{Loading}
			\\\hline\hline
			\textbf{PR Addition} & -0.49 \\
			\textbf{Deletion} & 0.52 \\
			\textbf{Files} & -0.52\\
			\textbf{PR Shared Files} & 0.81 \\
			\textbf{PR Deletion} & -0.84 \\
			\textbf{Addition} & 0.52 \\
			\textbf{PR Files} & 0.53 \\
			\textbf{Order} & -0.48 \\
			\hline
		\end{tabular}
		
	\end{center}		
\end{table}

==> tables/rosa_pr_performances.tex <==
\begin{table}[t]
	\begin{center}
		
		\caption{\szz's commit-set level performances - Perspective 3 (cases in the \rosab with both \bugin \& \bugout commits within commit-sets; N = 145)}
		\label{tab:szz_rosa_pr_performances}
		{\rowcolors{2}{LightCyan}{white}
		\begin{tabular}{|l|r|r|r|r|r|}
			\hline
			\textbf{Algorithm} & \textbf{Retrieved} & \textbf{Relevant} & \textbf{Prec.} & \textbf{Rec.} & \textbf{F1}
			\\\hline\hline
			\textbf{B-SZZ} & 230 & 74 & 0.32 & 0.38 & 0.35 \\
			\textbf{AG-SZZ} & 191 & 69 & 0.36 & 0.36 & 0.36 \\ 
			\textbf{L-SZZ} & 150 & 50 & 0.33 & 0.26 & 0.33 \\ 
			\textbf{R-SZZ} & 150 & 66 & 0.44 & 0.35 & 0.39 \\ 
			\textbf{Pydriller} & 222 & 75 & 0.33 & 0.39 & 0.36 \\ 
			\hline
		\end{tabular}
		}
		
	\end{center}		
\end{table}

==> tables/szz_commit_performances.tex <==
\begin{table}[t]
	\begin{center}
		
		\caption{\szz's commit-set level performance - Perspective~2 (cases in the \mozillab with a single commit on both \bugin and \bugout commit-sets; N = 1,596).}
		\label{tab:szz_commit_performances}
		{\rowcolors{2}{LightCyan}{white}
		\begin{tabular}{|l|r|r|r|r|r|}
			\hline
			\textbf{Algorithm} & \textbf{Retrieved} & \textbf{Relevant} & \textbf{Prec.} & \textbf{Rec.} & \textbf{F1}
			\\\hline\hline
			\textbf{B-SZZ} & 1,310 & 763 & 0.58 & 0.47 & 0.52 \\
			\textbf{AG-SZZ} & 1,236 & 620 & 0.50 & 0.38 & 0.43 \\ 
			\textbf{L-SZZ} & 1,245 & 470 & 0.37 & 0.29 & 0.33\\ 
			\textbf{R-SZZ} & 1,239 & 626 & 0.50 & 0.39 & 0.44\\ 
			\textbf{Pydriller} & 1,291 & 754 & 0.58 & 0.47 & 0.52 \\ 
			\hline
		\end{tabular}
		}
	\end{center}		
\end{table}
